Efficient Document Exchange and Error Correcting Codes with Asymmetric Information

We study two fundamental problems in communication, Document Exchange (DE) and Error Correcting Code (ECC). In the first problem, two parties hold two strings, and one party tries to learn the other party's string through communication. In the second problem, one party tries to send a message to another party through a noisy channel, by adding some redundant information to protect the message. Two important goals in both problems are to minimize the communication complexity or redundancy, and to design efficient protocols or codes. Both problems have been studied extensively. In this paper we study whether asymmetric partial information can help in these two problems. We focus on the case of Hamming distance/errors, and the asymmetric partial information is modeled by one party having a vector of disjoint subsets $\vec{S}=(S_1, \cdots, S_t)$ of indices and a vector of integers $\vec{k}=(k_1, \cdots, k_t)$, such that in each $S_i$ the Hamming distance/errors is at most $k_i$. We establish both lower bounds and upper bounds in this model, and provide efficient randomized constructions that achieve a $\min\lbrace O(t^2), O\left((\log \log n)^2\right) \rbrace $ factor within the optimum, with almost linear running time. We further show a connection between the above document exchange problem and the problem of document exchange under edit distance, and use our techniques to give an efficient randomized protocol with optimal communication complexity and \emph{exponentially} small error for the latter. This improves the previous result by Haeupler \cite{haeupler2018optimal} (FOCS'19) and that by Belazzougui and Zhang \cite{BelazzouguiZ16} (FOCS'16). Our techniques are based on a generalization of the celebrated expander codes by Sipser and Spielman \cite{sipser1996expander}, which may be of independent interests.

==> furtherreducingsketchlength.tex <==

We can further reduce the sketch size to $O(k \log \frac{n}{k})$ by applying the strategy "divide and conquer", while letting $k = \Omega(\log n)$.
That is, we apply a random hash function to divide the blocks in the current level to buckets each having $ n_i/\log n$ blocks. The division is uniform random s.t. bad blocks are almost evenly distributed into buckets.
Furthermore, bad blocks stemming from the same previous level, are also distributed evenly into these buckets. So for each group we can apply the target area decodable code.

\begin{construction}
\label{divideconcurmodifiedconstruct}


Replace the encoding step of level $i\in [L]$ with the following.

Let $R_j \in [ b ], j = 1,\ldots, m$ be a sequence  $\kappa = 0.01k/\log^2 n$-wise independent random variables, with $b = \Theta(\log n)$.

Alice's encoding:
\begin{itemize}

\item For $j\in [m]$, put message symbol $ x_{j} $ into set $ B[R_j] $;

\item Generate  $\Gamma_1: \{0,1\}^{l_i/b} \times \{0,1\}^{d_1 = 10} \rightarrow \{0, 1\}^{m_1 = O(k/b)}$ using randomness which is $O(k/\log n)$-wise independent (only generate $\Gamma_1$ once, reusing it in   future iterations);

\item Generate $\Gamma_2: \{0,1\}^{l_i/b} \times \{0,1\}^{d_2 = O((\log l_i) (\log k) )^{11}} \rightarrow \{0,1\}^{m_2 = O(k/b)}$ deterministically by Theorem \ref{expanderthm};

\item Apply encoding \ref{Enc:expandercode} on each $B[1], \ldots, B[b] $, using $\Gamma_1, \Gamma_2$;

\item Concatenate these encodings to be $z $.
\end{itemize}

Bob's decoding:
\begin{itemize}

\item For $j\in [m]$, put $\tilde{x}[j]$ into set $\tilde{B}[R_j] $;

\item For each $ r \in [b] $, 
\begin{itemize}
\item For every $ i'\in [i-1]$;
Let $S'_{i'} $ be the indices of the symbols that are put into bucket $r$, from $S_{i'}$;

\item Let $  \mathcal{S}'  = \{ {S}'_{i'}, i'\in [i-1]\}$;


\item Apply decoding \ref{constr:enhancedBPDec} on $\tilde{B}[r], \mathcal{S}', z, \Gamma_1, \Gamma_2$ to get $B[r]$;
\end{itemize}


 

\item Get $x$ from $B[1], \ldots, B[b] $.

\end{itemize}


\end{construction}

 

\begin{lemma}
\label{lem:randomnessused}
The randomness used has length $O(k \log \frac{n}{k})$.

\end{lemma}

\begin{proof}

The randomness used in generating $R_1, \ldots, R_{l_i}$, has length $O(k \log \frac{n}{k})$. The randomness used to generate $\Gamma_1$ has length $O(k)$. Note that randomness is reused for each time we need to generate $R_j, j\in [l_i], i\in [L]$ and  $\Gamma_1 $. 
%Also note that the randomness used to generate hash functions is also $O(k \log \frac{n}{k})$ since we use $2^{-\Omega(k)}$-almost $O(k)$-wise independence generator. 

So the total randomness used has length $O(k \log \frac{n}{k})$.

\end{proof}


Next we show that this modified encoding/decoding can work as well as the original one.
\begin{lemma}
\label{lem:divideconcurcomputingx}

For every $k\in \mathbb{N}$, every $S_{i'} \subseteq [m], {i'}\in [i-1]$ be s.t. $|S_{i'}| = \Theta(2^{i-{i'}} k)$, let $k_{i'} = \max(k/2^{c(i-{i'})}, k_0) , {i'}\in [i-1]$, be the number of errors in $ S_{i'} $.

With probability $1-2^{-\Omega(k^{0.9})}$, the decoding can compute $x$ correctly.

\end{lemma}

\begin{proof}
Consider an arbitrary  $ r \in [b]$. 
%Let $S'_j $ be the indices of the symbols that are put into bucket $r$, from $S_j$.
Let $Y = \sum_{s \in S_{i'}} Y_{s} $, where $Y_s$ indicates that $s$ is in the bucket. Note that $\mathbb{E}Y = |S_{i'}|/b$.

By Theorem \ref{kwiseconcentrbound},
$$ \Pr[  Y-\mathbb{E}Y  \geq 0.5\mathbb{E}Y   ] \leq  2^{-\Omega(\kappa)}. $$

Hence, with probability $1-2^{-\Omega(\kappa)}$, $Y \leq 1.5|S_{i'}|/b$.


Similarly, the number of errors in $S_{i'}$ that are put into bucket $r$, denoted by $k'_{i'}$, is at most $ 1.5k_{i'}/b $ with probability at least $1-2^{-\Omega(\kappa)}$.

By a union bound, with probability $1- i b 2^{\Omega(\kappa)} \geq 1-2^{\Omega(\kappa)}$ for every bucket $r$, for every ${i'}$, 
\begin{itemize}
\item the number of elements in $S_{i'}$ is put into bucket $r$ is at most $1.5|S_{i'}|/b$;

\item the number of wrongly recovered symbols in $S_{i'}$ that are put into bucket $r$ is at most $1.5k_{i'}/b$.

\end{itemize}
 
Consider bucket $r$.
By Lemma \ref{lem:expanderGeneration}, with probability at least $1-2^{-\Omega(k^{0.9})}$, $\Gamma_1$ is a $(  1.5k/b, (1.5k/b)^{0.9}, O(1) )$-target area expander.   By Lemma \ref{lem:enhancedBPDec}, the decoding can output the bits of $x$ in bucket $r$ correctly.   

By a union bound, the overall success probability for decoding all buckets correctly is at least $1-2^{-\Omega(k^{0.9})}$.



\end{proof}


\begin{theorem} \label{thm:OWProtocol}
	There exists a randomized one-way document exchange protocol, for every $k = \Omega(\log^{1.2} \frac{n}{k})$, with sketch size $O(k \log \frac{n}{k})$,   success  probability $1 -   2^{-\Omega(k^{0.9})}$, running time .
\end{theorem}

\begin{proof}
By Lemma \ref{lem:randomnessused}, we can further reduce the randomness used to $O(k \log \frac{n}{k})$. We let Alice send the randomness at the beginning of the protocol. So the randomness sent has length $O(k\log \frac{n}{k})$. After   Bob received the randomness, the communication complexity for remaining operations is $O(k\log \frac{n}{k})$ by Lemma \ref{lem:OWCC}. So the overall communication complexity is as stated.




By Lemma \ref{lem:divideconcurcomputingx}, Bob can correctly compute $x$.

By Lemma  \ref{lem:OWTimeC}, Construction \ref{Constr:OWDocExc} runs in polynomial time. Note that in our modified construction,  \ref{divideconcurmodifiedconstruct}, the protocol generates   expander graphs $\Gamma_1, \Gamma_2$ and applying the encoding/decoding from Construction \ref{Enc:expandercode} and \ref{constr:enhancedBPDec}. These are all in polynomial time so the overall running time is polynomial.

 


\end{proof}

==> multiround.tex <==
\section{Construction}
In this section we prove the following theorem.

\begin{theorem} \label{thm:multiround}
	There exists a randomized $O(\log \frac{n}{k})$-round document exchange protocol with sketch size $O(k \log \frac{n}{k})$, and sucessful probability $1 - 2^{-\Omega(k^{0.1})}$, for any $k = \Omega(\log^{1.1} n)$.
\end{theorem}

\begin{construction}
	Let $n$ be the length of the string. For $l \in [\lfloor \log\frac{n}{k} \rfloor]$, $T_l = \frac{n}{ 2^{l-1}k}$. For $j = 1, 2, \dots \lfloor \log_{2.1} k \rfloor$, denote $k_j = \frac{k}{2.1^j} \cdot 2^j$. For simplicity, we assume $n$ is a multiple of $2^{l-1} k$ and a multiple of $T_l$.
	
	Alice : input a binary string $x$ of length $n$.
	
	Bob : input a binary string $y$ of length $n'$, $\mathsf{ED}(x, y) \le k$.
	
	Bob creates an empty string $x'$ of length $n$. He will gradually fill $x'$ until it equals to $x$.
	
	The protocol runs in $\lfloor \log\frac{n}{k} \rfloor$ levels. 
	In each level, Alice sends a message to Bob, then Bob sends a message back to Alice.
	
	For $l$-th level, $l = 1, 2, \cdots, \lfloor \log\frac{n}{k} \rfloor$, Alice does the following:
	
	(Alice Phase I)	
	\begin{enumerate}
		\item Partition her string $x$ into $n_l$ blocks of size $T_l$, i.e. $x = x[1, T_l] \circ x(T_l, 2T_l] \circ \cdots \circ x((n_l - 1) T_l, n]$. Then generate a series of random hash functions $\phi_1, \phi_2, \cdots, \phi_{n_l}$, and $\varphi_1, \varphi_2, \cdots, \varphi_{n_l}$, each of them is a map $\{0, 1\}^{T_l} \rightarrow [c']$. If $l = \lfloor \log \frac{n}{k} \rfloor$, i.e., the last level, then $T_l = O(1)$, and let $(\phi_i)_{i\in n_l}$ be the identity functions.
		
		\item If $l = 1$, then mark each block as ``ancestor''.
		If $l \ge 2$, then iterate all blocks $i \in [n_l]$. For $i$-th block $x((i-1)T_l+1, i T_l]$. Find the first block marked as ``ancester'' in its father and grandfather etc. If such ancester is in $l-1, l-2, \cdots, \max(l-\lfloor \log_{2.1} k\rfloor, 1) $-th level,  then denote the substring in this block as $a_i$, otherwise let $a_i$ be an empty string.
		Let $V[i] = (\phi_i(x((i-1)T_l+1, i T_l]), \varphi_i(a_i))$, where $a_i$ is padded to the length $T_l$.
		
		\item For $j = 1, 2, \cdots, \min(\lfloor \log_{2.1} k) \rfloor, l-1)$, we construct a set $S_j$ as follows. Initially $S_j$ is empty. 
		Iterate on all blocks in $(l-j)$-th level.
		For each $u \in [n_{l-j}]$, if $u$-th block $x((u-1)T_{l-j}, u T_{l-j}]$ is marked as ``ancestor'', and all its descendants is not marked ``ancestor'', then we add all its $2^j$ descendants blocks in $l$-th level : $\{ (u-1)2^j+1, (u-1)2^j+2, \cdots, u 2^j \}$ into $S_j$. Denote $v_{l, j} = (V[w])_{w \in S_j}$. 
		Send a redundancy $\mathsf{sk}_{l, j}$ of $v_{l, j}$ being able to correct $k_j$ errors using Theorem~\ref{thm:algebraic-geometry-code}.
	\end{enumerate}
	
	Bob receives the sketches $(\mathsf{sk}_{l,j})_j$, and does the following:
	\begin{enumerate}
		\item Partition string $x'$ into $n_l$ blocks of size $T_l$, i.e. $x' = x'[1, T_l] \circ x'(T_l, 2T_l] \circ \cdots \circ x'((n_l-1) T_l, n]$. Then use the same randomness with Alice to generate the hash functions $\phi_1, \phi_2, \cdots, \phi_{n_l}$, and $\varphi_1, \varphi_2, \cdots, \varphi_{n_l}$.
		
		\item If $l = 1$, then mark each block as ``ancestor''. 
		If $l \ge 2$, then
		for $i$-th block $x'[(i-1)T_l+1, i T_l)$, find the first block marked as ``ancester'' in its father and grandfather etc. If such ancester is in $l-1, l-2, \cdots, \max(l-\lfloor \log_{2.1} k\rfloor, 1) $-th level, then denote the substring in this block as $a_i'$, otherwise let $a_i'$ be an empty string.
		For each $i \in [n_l]$, Let $V'[i] = (\phi_i(x'((i-1)T_l+1, i T_l]), \varphi_i(a_i'))$, where $a_i'$ is padded to the length $T_l$.
		
		\item For $j = 1, 2, \cdots, \min(\lfloor \log_{2.1} k \rfloor, l-1)$, we construct a set $S_j$ as follows. Initially $S_j$ is empty. 
		Iterate on all blocks in level $l-j$.
		For each $u \in [n_{l-j}']$, if $u$-th block $x((u-1)T_{l-j}, u T_{l-j}]$ is marked as ``ancestor'', and all its descendants is not marked ``ancestor'', then we add all its $2^j$ descendants blocks in $i$-th level $\{ (u-1)2^j+1, (u-1)2^j+2, \cdots, u 2^j \}$ to $S_j$. Denote $v_{l, j}' = (V'[w])_{w \in S_j}$. Then we use $\mathsf{sk}_{l, j}$ and $v'_{l,j}$ to recover Alice's $v_{l,j}$. For all $w \in S_j$, Bob sets $V''[w] = v_{l, j}[w]$.
		
		\item For each $i \in \cup_{j} S_j$, if $V'[i] \neq V''[i]$, let the ancestor of $i$ be the block $b$ in $(l - j)$-th level such that $j \le \lfloor \log_{2.1} k \rfloor$.
		If such ancestor $b$ exists, 
		we rematch the hash values of $2^j$ descendants of $b$ between $y$ under the hash functions $(\phi_i)_i$. For each unmatched descendant block, we fill the block using random strings.
		Then we mark each descendants as ``ancestor''.
		
		\item For each $j = 1, 2, \cdots, \min(\lfloor \log_{2.1} k \rfloor, l-1)$, compute a sketch $\mathsf{sk}_{l, j}'$ of $(V'[w])_{w \in S_j}$ being able to correct $k_j$ errors, and send $\mathsf{sk}_{l,j}'$ to Alice.
	\end{enumerate}
	
	Alice receives the sketches $(\mathsf{sk}_{l,j}')_j$, and does the following.
	
	(Alice Phase II)
	\begin{enumerate}
		\item For each $j = 1, 2, \cdots, \min(\lfloor \log_{2.1} k \rfloor, l-1)$, use $\mathsf{sk}_{l, j}'$ and $(V[w])_{w \in S_j}$ to recover Bob's $(V'[w])_{w \in S_j}$.
		For every $w\in S_j$, if $V'[w] \neq V[w]$,
		then mark $w$-th block as ``ancestor''.
	\end{enumerate}
\end{construction}


\begin{lemma}\label{lemma:ancestor}
	For $l = 1, 2, \cdots,  \lfloor \log\frac{n}{k} \rfloor$, in $l$-th level, the following properties holds with probability $1 - 2^{-\Omega(k^{0.1})}$.
	
	\begin{enumerate}
		
		\item The number of blocks marked as ``ancestor'' is bounded by $10 k$ in both Alice's and Bob's side.
		
		\item For each $j = 1, 2, \cdots, \min(\lfloor \log_{2.1} k \rfloor, l-1)$, 
		the number of undetected incorrectly filled ancestors in $(l - j)$-th level is at most $\frac{k}{2.1^j}$. Hence, the Hamming distance between $(V'[w])_{w \in S_j}$ and $(V[w])_{w \in S_j}$ is $k_j = \frac{k}{2.1^j}\cdot 2^j $.
	\end{enumerate}
\end{lemma}

\begin{proof}
	We prove this lemma by induction on the levels. For the first level, since we mark all blocks in the first level as ``ancestor'', the lemma holds. 
	Now we assume the lemma holds for the first $l$ levels, and prove for the lemma in $(l+1)$-th level.
	
	We now prove Property 1. The $i$-th block in $(l+1)$-th level is marked as ``ancestor'', if $V'[i] \neq V[i]$. %Note that in Bob's side, he only recovers the values for $(V[w])_{w \in S_j}$, for $j = 1, 2, \cdots, \lfloor \log_{2.1} k \rfloor$. 
	For each such block, we find the lowest ``ancestor'' in its father, grandfather, etc.
	Now there are two cases: 
	1. the ancestor is in the first $\min(l - \lfloor \log_{2.1} k \rfloor, 1)-1$ levels.
	2. the ancestor is in $l-1, l-2, \min(l - \lfloor \log_{2.1} k \rfloor, 1)$-th level. 
	
	For the first case, since the incorrectly filled ancestor is checked by $2^{\lfloor \log_{2.1} k \rfloor}$ hashes, this happens with probability $c'^{-2^{\lfloor \log_{2.1} k \rfloor}} \le 2^{-k^{\frac{1}{\log 2.1}}} \le 2^{-k^{0.9}}$.
	By a union bound on all levels, the probability of case 1 for at least one level is bounded by $ O(\log n) / 2^{k^{0.9}}$. When $k = \Omega(\log^{1.1} n)$, this probability is at most $2^{-\Omega(k^{0.9})}$. 
	
	For the second case, by the induction hypothesis, the number of such ancestors is $k / 2.1^{j-1}$, and each of them has $2^j$ descendents. Hence, the total number of ancestors in $l$-th level is at most $\sum_{j=0}^{\lfloor \log_{2.1} k \rfloor} \frac{k}{2.1^{j-1}} \cdot 2^j \le 10 k$.
	
	Next, we prove Property 2. From Property 1 on all previous levels, let the number of undetected incorrectly filled ancestors in $(l-j)$-th level be $k_j'$, then
	$\Pr[k_j > k_j'] = \Pr[\sum_{u \in [10k]} b_u  > k_j']$, where each $b_u$ is a Bernoulli variable with $\Pr[b_u = 1] = c'^{-2^j}$. Applying the Chernoff bound, we obtain $\Pr[\sum_{u \in [10k]} b_u  > k_j'] < 2^{-\Omega(k^{0.1})}$. By a union bound on all levels, the probability of case 2 is at most $\log n \log k / 2^{\Omega(k^{0.1})}$. When $k = \Omega(\log^{1.1} n)$, this probability is $2^{-\Omega(k^{0.1})}$.
\end{proof}

\begin{proof}[Proof of Theorem~\ref{thm:multiround}]
By Property 2 in Lemma~\ref{lemma:ancestor}, Bob uses the sketches $(\mathsf{sk}_{l, j})_j$ and his $V'$ to recover Alice's $V$ correctly. 
Alice also recovers Bob's $V'$ correctly. 
For each $l$, in $l$-th level, the length of the sketches is $\sum_{j} |\mathsf{sk}_{l, j}| = \sum_{j} k_j \log \frac{|S_j|}{k_j}$. 
From Property 1 in Lemma~\ref{lemma:ancestor}, 
we put at most $10k 2^j$ elements in $S_j$. 
Hence, $|S_j| \le 10 k 2^j$. 
We obtain 
\begin{align}
\sum_{j}^{\lfloor \log_{2.1} k \rfloor} k_j \log \frac{|S_j|}{k_j} = \sum_{j}^{\lfloor \log_{2.1} k \rfloor} k(\frac{2}{2.1})^j \log\frac{10k 2^j}{k (2/2.1)^j} = \sum_{j}^{\lfloor \log_{2.1} k \rfloor} k (\frac{2}{2.1})^j \cdot j \cdot O(1) = O(k)
\end{align} 
Since we have $O(\log \frac{n}{k})$ levels, the total sketch size is $O(k \log \frac{n}{k})$.
\end{proof}
